Demystifying Invariant Effectiveness for Securing Smart Contracts

Smart contract transactions associated with security attacks often exhibit distinct behavioral patterns compared with historical benign transactions before the attacking events. While many runtime monitoring and guarding mechanisms have been proposed to validate invariants and stop anomalous transactions on the fly, the empirical effectiveness of the invariants used remains largely unexplored. In this paper, we studied 23 prevalent invariants of 8 categories, which are either deployed in high-profile protocols or endorsed by leading auditing firms and security experts. Using these well-established invariants as templates, we developed a tool Trace2Inv which dynamically generates new invariants customized for a given contract based on its historical transaction data. We evaluated Trace2Inv on 42 smart contracts that fell victim to 27 distinct exploits on the Ethereum blockchain. Our findings reveal that the most effective invariant guard alone can successfully block 18 of the 27 identified exploits with minimal gas overhead. Our analysis also shows that most of the invariants remain effective even when the experienced attackers attempt to bypass them. Additionally, we studied the possibility of combining multiple invariant guards, resulting in blocking up to 23 of the 27 benchmark exploits and achieving false positive rates as low as 0.32%. Trace2Inv outperforms current state-of-the-art works on smart contract invariant mining and transaction attack detection in terms of both practicality and accuracy. Though Trace2Inv is not primarily designed for transaction attack detection, it surprisingly found two previously unreported exploit transactions, earlier than any reported exploit transactions against the same victim contracts.

==> sections/acknowledgement.tex <==
% \section*{Acknowledgement}



==> sections/dataAvailability.tex <==

% \section{Data Availability}
% The experimental data of this paper is available on our website~\cite{website}.


==> tables/RQ2.tex <==
% \vspace{-3mm}
\begin{table}[h]
    \scriptsize
    \caption{Bypassability Results of True Positives and Sampled False Positives}
    \label{tab:bypass}
    \scriptsize
    \tabcolsep=0.11cm


    \begin{tabular}{l|l|lllll|lll|ll|l|ll|ll|llll|llll}
                                                &    & \multicolumn{5}{c}{Access Control}                    & \multicolumn{3}{c}{Time Lock}  & \multicolumn{2}{c}{Gas Control} & \multicolumn{1}{c}{Re} & \multicolumn{2}{c}{Oracle} & \multicolumn{2}{c}{Storage} & \multicolumn{4}{c}{Data Flow}                 & \multicolumn{4}{c}{Money Flow}                   \\
                                                &    & \rot{EOA} & \rot{SO} & \rot{SM} & \rot{OO} & \rot{OM} & \rot{SB} & \rot{OB} & \rot{LU} & \rot{GS}       & \rot{GC}       & \rot{RE}               & \rot{OR}     & \rot{OD}    & \rot{TSU}    & \rot{TBU}    & \rot{MU} & \rot{CVU} & \rot{DFU} & \rot{DFL} & \rot{TIU} & \rot{TOU} & \rot{TIRU} & \rot{TORU} \\   \toprule
    \multirow{5}{*}{True Positives}             & C1 & 9         & 5        & 7        & 4        & 9        & 2        & 6        & 1        & 0              & 23             & 2                      & 5            & 4           & 2            & 7            & 1        & 0         & 0         & 1         & 0         & 0         & 0          & 0          \\
                                                & C2 & 14        & 0        & 0        & 0        & 0        & 0        & 6        & 5        & 0              & 0              & 0                      & 0            & 0           & 0            & 0            & 0        & 1         & 13        & 0         & 7         & 14        & 2          & 8          \\
                                                & C3 & 0         & 0        & 0        & 0        & 0        & 0        & 1        & 1        & 0              & 0              & 0                      & 0            & 0           & 0            & 0            & 0        & 1         & 1         & 0         & 2         & 1         & 0          & 0          \\
                                                & C4 & 0         & 0        & 0        & 0        & 0        & 0        & 0        & 0        & 1              & 0              & 0                      & 2            & 0           & 6            & 5            & 0        & 0         & 0         & 0         & 0         & 0         & 2          & 14         \\
                                                & C5 & 0         & 0        & 0        & 0        & 0        & 9        & 0        & 5        & 29             & 0              & 0                      & 0            & 0           & 0            & 0            & 0        & 0         & 9         & 0         & 0         & 7         & 1          & 0          \\  \midrule
    \multirow{3}{*}{False Positives}            & D1 & 10        & 10       & 10       & 10       & 10       & 0        & 0        & 1        & 0              & 10             & 0                      & 10           & 10          & 10           & 10           & 10       & 0         & 4         & 10        & 0         & 0         & 0          & 1          \\
                                                & D2 & 0         & 0        & 0        & 0        & 0        & 0        & 0        & 0        & 0              & 0              & 0                      & 0            & 0           & 0            & 0            & 0        & 8         & 6         & 0         & 10        & 10        & 10         & 9          \\
                                                & D3 & 0         & 0        & 0        & 0        & 0        & 0        & 0        & 9        & 10             & 0              & 0                      & 0            & 0           & 0            & 0            & 0        & 0         & 0         & 0         & 0         & 0         & 0          & 0          \\   \bottomrule
    \end{tabular}

    \vspace{-3mm}
    \end{table}

==> tables/benchmarks.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \vspace{-3mm}
\begin{table}[!htbp]
    \scriptsize
    \caption{Benchmarks$^{+}$. (\textbf{Exploit:} the first exploit transaction during the incident. \textbf{FL:} whether the exploit transaction uses flash loan. 
     \textbf{Contracts:} the victim contracts involved in the exploit. \textbf{Type:} the type of the contract, either interface (I) or payload (P).  \textbf{PL:} the programming language of the contract, either Solidity (S) or Vyper (V). 
     \textbf{History:} the number of transactions in the history of the contract up to the exploit transaction.)}
     \vspace{-3mm}
     \label{tab:benchmarks}
    
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
    \hline
    \slide{Kind}                                                             & Victim Protocol                 & Root Cause                                                                             & Date                      & Loss                   & Exploit                                                               &   FL                              & Contracts          & Type & PL  & History \\ \hline
    \multirow{4}{*}{\vertical{Bridges}}                                      & RoninNetwork                    & keys compromised                                                                       & 22/03/29                  & 624M                   & \cite{RoninNetwork}                                                   &                                   & RoninNetwork       & I+P  & S   & 95345   \\ \cline{2-11} 
                                                                             & HarmonyBridge                   & keys compromised                                                                       & 22/06/24                  & 100M                   & \cite{HarmonyBridge}                                                  &                                   & HarmonyBridge      & P    & S   & 32149   \\ \cline{2-11} 
                                                                             & Nomad                           & \begin{tabular}[c]{@{}l@{}}zero hash as \\ a valid root\end{tabular}                   & 22/08/01                  & 152M                   & \cite{Nomad}                                                          &                                   & Nomad              & I+P  & S   & 15630   \\ \cline{2-11} 
                                                                             & PolyNetwork                     & hash collision                                                                         & 21/08/10                  & 611M                   & \cite{PolyNetwork}                                                    &                                   & PolyNetwork        & I+P  & S   & 44509   \\ \hline
    \multirow{19}{*}{\vertical{Lending}}                                     & bZx2                            & oracle manipulation                                                                    & 20/02/18                  & 630K                   & \cite{bZx2}                                                           &  \cmark                           & bZx2               & I+P  & S   & 711     \\ \cline{2-11} 
                                                                             & \multirow{2}{*}{Warp}           & \multirow{2}{*}{oracle manipulation}                                                   & \multirow{2}{*}{20/12/17} & \multirow{2}{*}{8M}    &                                                                       &                                   & Warp               & P    & S   & 148     \\ 
                                                                             &                                 &                                                                                        &                           &                        & \multirow{-2}{*}{\cite{Warp}}                                         &  \multirow{-2}{*}\cmark           & Warp\_I            & I    & S   & 31      \\ \cline{2-11} 
                                                                             & \multirow{3}{*}{CheeseBank}     & \multirow{3}{*}{oracle manipulation}                                                   & \multirow{3}{*}{20/11/06} & \multirow{3}{*}{3.3M}  &                                                                       &                                   & CheeseBank\_1      & I+P  & S   & 615     \\ 
                                                                             &                                 &                                                                                        &                           &                        &                                                                       &                                   & CheeseBank\_2      & I+P  & S   & 593     \\  
                                                                             &                                 &                                                                                        &                           &                        & \multirow{-3}{*}{\cite{CheeseBank}}                                   &  \multirow{-3}{*}\cmark           & CheeseBank\_3      & I+P  & S   & 557     \\ \cline{2-11} 
                                                                             & InverseFi                       & oracle manipulation                                                                    & 22/06/16                  & 1.26M                  & \cite{InverseFi}                                                      &  \cmark                           & InverseFi          & I+P  & S   & 7590    \\ \cline{2-11} 
                                                                             & \multirow{2}{*}{CreamFi1}       & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}cross contract\\ re-entrancy\end{tabular}}  & \multirow{2}{*}{21/08/30} & \multirow{2}{*}{18M}   &                                                                       &                                   & CreamFi1\_1        & I+P  & S   & 5       \\  
                                                                             &                                 &                                                                                        &                           &                        & \multirow{-2}{*}{\cite{CreamFi1}}                                     &  \multirow{-2}{*}\cmark           & CreamFi1\_2        & I+P  & S   & 58184   \\ \cline{2-11} 
                                                                             & \multirow{4}{*}{CreamFi2}       & \multirow{4}{*}{oracle manipulation}                                                   & \multirow{4}{*}{21/10/27} & \multirow{4}{*}{130M}  &                                                                       &                                   & CreamFi2\_1        & I+P  & S   & 1270    \\  
                                                                             &                                 &                                                                                        &                           &                        &                                                                       &                                   & CreamFi2\_2        & I+P  & S   & 898     \\ 
                                                                             &                                 &                                                                                        &                           &                        &                                                                       &                                   & CreamFi2\_3        & I+P  & S   & 261     \\ 
                                                                             &                                 &                                                                                        &                           &                        & \multirow{-4}{*}{\cite{CreamFi2}}                                     &  \multirow{-4}{*}\cmark           & CreamFi2\_4        & I+P  & S   & 98      \\ \cline{2-11} 
                                                                             & RariCapital1                    & read-only re-entrancy                                                                  & 21/05/09                  & 10M                    & \cite{RariCapital1}                                                   &  \cmark                           & RariCapital1       & I+P  & S   & 667     \\ \cline{2-11} 
                                                                             & \multirow{4}{*}{RariCapital2}   & \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}cross contract\\ re-entrancy\end{tabular}}  & \multirow{4}{*}{22/04/30} & \multirow{4}{*}{80M}   &                                                                       &                                   & RariCapital2\_1    & I+P  & S   & 614     \\ 
                                                                             &                                 &                                                                                        &                           &                        &                                                                       &                                   & RariCapital2\_2    & I+P  & S   & 752     \\ 
                                                                             &                                 &                                                                                        &                           &                        &                                                                       &                                   & RariCapital2\_3    & I+P  & S   & 404     \\  
                                                                             &                                 &                                                                                        &                           &                        & \multirow{-4}{*}{\cite{RariCapital2}}                                 & \multirow{-4}{*}\cmark            & RariCapital2\_4    & I+P  & S   & 776     \\ \cline{2-11} 
                                                                             & XCarnival                       & logic error                                                                            & 22/06/26                  & 3.87M                  & \cite{XCarnival}                                                      &                                   & XCarnival          & I+P  & S   & 342     \\ \hline
    \multirow{8}{*}{\vertical{Yield-Earning}}                                & Harvest1                        & oracle manipulation                                                                    & 20/10/26                  & \multirow{2}{*}{33.8M} & \cite{Harvest1}                                                       & \cmark                            & Harvest1           & I+P  & S   & 2050    \\ \cline{2-4} \cline{6-11} 
                                                                             & Harvest2                        & oracle manipulation                                                                    & 20/10/26                  &                        & \cite{Harvest2}                                                       & \cmark                            & Harvest2           & I+P  & S   & 2161    \\ \cline{2-11} 
                                                                             & ValueDeFi                       & oracle manipulation                                                                    & 20/11/14                  & 7.4M                   & \cite{ValueDeFi}                                                      & \cmark                            & ValueDeFi          & I+P  & S   & 295     \\ \cline{2-11} 
                                                                             & \multirow{2}{*}{Yearn}          & \multirow{2}{*}{forced investment}                                                     & \multirow{2}{*}{21/02/04} & \multirow{2}{*}{11M}   &                                                                       &                                   & Yearn              & P    & S   & 672     \\ 
                                                                             &                                 &                                                                                        &                           &                        & \multirow{-2}{*}{\cite{Yearn}}                                        & \multirow{-2}{*}\cmark            & Yearn\_I           & I    & S   & 26688   \\ \cline{2-11} 
                                                                             & VisorFi                         & re-entrancy                                                                            & 21/12/21                  & 8.2M                   & \cite{VisorFi}                                                        &                                   & VisorFi            & I+P  & S   & 1693    \\ \cline{2-11} 
                                                                             & UmbrellaNetwork                 & underflow bug                                                                          & 22/03/20                  & 700K                   & \cite{UmbrellaNetwork}                                                &                                   & UmbrellaNetwork    & I+P  & S   & 59      \\ \cline{2-11} 
                                                                             & PickleFi                        & access control                                                                         & 20/11/21                  & 20M                    & \cite{PickleFi}                                                       &                                   & PickleFi           & I+P  & S   & 5439    \\ \hline
    \multirow{11}{*}{\vertical{Others}}                                      & Eminence                        & logic error                                                                            & 20/09/29                  & 7M                     & \cite{Eminence}                                                       &  \cmark                           & Eminence           & I+P  & S   & 20589   \\ \cline{2-11} 
                                                                             & Opyn                            & logic error                                                                            & 20/08/04                  & 371k                   & \cite{Opyn}                                                           &                                   & Opyn               & I+P  & S   & 67      \\ \cline{2-11} 
                                                                             & IndexFi                         & logic error                                                                            & 21/10/15                  & 16M                    & \cite{IndexFi}                                                        &  \cmark                           & IndexFi            & I+P  & S   & 20641   \\ \cline{2-11} 
                                                                             & \multirow{2}{*}{RevestFi}       & \multirow{2}{*}{re-entrancy}                                                           & \multirow{2}{*}{22/03/27} & \multirow{2}{*}{11.2M} &                                                                       &                                   & RevestFi           & P    & S   & 1635    \\ 
                                                                             &                                 &                                                                                        &                           &                        & \multirow{-2}{*}{\cite{RevestFi}}                                     &  \multirow{-2}{*}\cmark           & RevestFi\_I        & I    & S   & 1463    \\ \cline{2-11} 
                                                                             & DODO                            & access control                                                                         & 21/03/08                  & 700K                   & \cite{DODO}                                                           &  \cmark                           & DODO               & I+P  & S   & 42      \\ \cline{2-11} 
                                                                             & \multirow{3}{*}{Punk}           & \multirow{3}{*}{access control}                                                        & \multirow{3}{*}{21/08/10} & \multirow{3}{*}{8.9M}  &                                                                       &                                   & Punk\_1            & I+P  & S   & 28      \\ 
                                                                             &                                 &                                                                                        &                           &                        &                                                                       &                                   & Punk\_2            & I+P  & S   & 42      \\ 
                                                                             &                                 &                                                                                        &                           &                        & \multirow{-3}{*}{\cite{Punk}}                                         &                                   & Punk\_3            & I+P  & S   & 37      \\ \cline{2-11} 
                                                                             & \multirow{2}{*}{BeanstalkFarms} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}flashloan assisted\\ commit\end{tabular}}   & \multirow{2}{*}{22/04/16} & \multirow{2}{*}{182M}  &                                                                       &                                   & BeanstalkFarms     & P    & V   & 5785    \\ 
                                                                             &                                 &                                                                                        &                           &                        & \multirow{-2}{*}{\cite{BeanstalkFarms}}                               & \multirow{-2}{*}\cmark            & BeanstalkFarms\_I  & \revise{I} & \revise{S}    & 306    \\ \hline
    \end{tabular}
    \flushleft
    \scriptsize
    \camera{$^+$: All contracts and transactions within these benchmarks can be found at~\cite{benchmarks}}.
    \vspace{-4mm}
    \end{table}


==> tables/calltreeOpcodes.tex <==
\begin{table}[!htbp]
    \caption{EVM Opcodes Used to Construct Invocation Tree}
    \label{tab:calltreeOpcodes}
    \scriptsize
    \begin{tabular}{|l|l|}
    \hline
                    & EVM opcodes                                               \\ \hline
    Function Enter & call, callcode, staticcall, delegatecall, create, create2 \\ \hline
    Function Exit  & stop, return, revert, selfdestruct, (out of gas)          \\ \hline
    \end{tabular}
    \vspace{-4mm}
    \end{table}


==> tables/evmopcodes.tex <==
\begin{table}[h]

    \scriptsize
    \caption{EVM Opcodes Grouped by Category}
    \begin{tabular}{|l|l|}
    \hline
        Category                       & EVM opcodes                                                                                                                      \\ \hline
        External Address Variables  & balance, extcodesize, extcodecopy, extcodehash,                                                                                     \\ \hline
        Execution Context Variables & origin, caller, address, codesize, selfbalance, pc, msize, gas                                                                      \\ \hline
        Call Data Variables         & callvalue, calldataload, calldatasize, calldatacopy                                                                                 \\ \hline
        Return Data Variables       & returndatasize, returndatacopy                                                                                                      \\ \hline
        Block Properties            & blockhash, coinbase, timestamp, number, prevrandao, gasprice, gaslimit, chainid,                                                    \\ \hline
        Stack Operations            & pop, push1-push32, dup1-dup16, swap1-swap16                                                                                         \\ \hline
        Memory Operations           & mload, mstore, mstore8                                                                                                              \\ \hline
        Storage Operations          & sload, sstore                                                                                                                       \\ \hline
        Logical Operations          & lt, gt, slt, sgt, eq, iszero, and, or, xor, not, byte, shl, shr, sar                                                                \\ \hline
        Cryptographic Operations    & sha3                                                                                                                                \\ \hline
        Arithmetic Operations       & add, mul, sub, div, sdiv, mod, smod, addmod, mulmod, exp,                                                                           \\ \hline
        Logging Operations          & log0-log4                                                                                                                           \\ \hline
        Contract Call               & call, callcode, staticcall, delegatecall                                                                                            \\ \hline
        Contract Return             & stop, return, revert                                                                                                                \\ \hline
        Contract Creation           & create, create2                                                                                                                     \\ \hline
        Contract Destruction        & selfdestruct                                                                                                                        \\ \hline
    \end{tabular}
    \end{table}


==> tables/invariants1.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
    \scriptsize

    \caption{Invariants}
    \label{tab:invariants}
    
    \begin{tabular}{|l|l|l|l|l|l|}
    \hline
    Category                         & ID   & Name                    & Parameter to learn & Sources                     & Related Opcodes                                   \\ \hline
    \multirow{5}{*}{Access Control}  & EOA  & onlyEOA                 &                    & \multirow{5}{*}{literature} & origin, sender                                    \\ \cline{2-4} \cline{6-6} 
                                     & SO   & isSenderOwner           & Address            &                             & sender                                            \\ \cline{2-4} \cline{6-6} 
                                     & SM   & isSenderManager         & Set of Address     &                             & sender                                            \\ \cline{2-4} \cline{6-6} 
                                     & OO   & isOriginOwner           & Address            &                             & origin                                            \\ \cline{2-4} \cline{6-6} 
                                     & OM   & isOriginManager         & Set of Address     &                             & origin                                            \\ \hline
    \multirow{3}{*}{Time Lock}       & SB   & isSameSenderBlock       &                    & \multirow{2}{*}{1}          & sender, block(*)                                  \\ \cline{2-4} \cline{6-6} 
                                     & OB   & isSameOriginBlock       &                    &                             & origin, block(*)                                  \\ \cline{2-6} 
                                     & LU   & lastUpdate              & Integer            & 2,3                         & block(**)                                         \\ \hline
    Re-entrancy                      & RE   & nonReEntrant            &                    & literature                  &                                                   \\ \hline
    \multirow{2}{*}{Gas Control}     & GS   & GasStartUpperBound      & Integer            & \multirow{2}{*}{motivated}  & gas                                               \\ \cline{2-4} \cline{6-6} 
                                     & GC   & GasConsumedUpperBound   & Integer            &                             & gas                                               \\ \hline
    \multirow{2}{*}{Oracle Slippage} & OR   & OracleRange             & Integer            & 6                           & call(*)                                           \\ \cline{2-6} 
                                     & OD   & OracleDeviation         & Integer            & literature                  & call(*)                                           \\ \hline
    \multirow{2}{*}{Special Storage} & TSU  & TotalSupplyUpperBound   & Integer            & 4, 7                        & sload, sstore                                     \\ \cline{2-6} 
                                     & TBU  & TotalBorrowUpperBound   & Integer            & 4, 7                        & sload, sstore                                     \\ \hline
    \multirow{4}{*}{Data Flow}       & MU   & MappingUpperBound       & Integer            &                             & sload, sha3                                       \\ \cline{2-6} 
                                     & CVU  & CallValueUpperBound     & Integer            &                             & callvalue                                         \\ \cline{2-6} 
                                     & DFU  & DataFlowUpperBound      & Integer            &                             & calldata(*), sload, balance, call(*), selfbalance \\ \cline{2-6} 
                                     & DFL  & DataFlowLowerBound      & Integer            &                             & calldata(*), sload, balance, call(*), selfbalance \\ \hline
    \multirow{4}{*}{Money Flow}      & TIU  & TokenInUpperBound       & Integer            & 7                           & call(*)                                           \\ \cline{2-6} 
                                     & TIRU & TokenInRatioUpperBound  & Integer            & motivated                   & call(*)                                           \\ \cline{2-6} 
                                     & TIL  & TokenOutUpperBound      & Integer            & 8                           & call(*)                                           \\ \cline{2-6} 
                                     & TIRU & TokenOutRatioUpperBound & Integer            & motivated                   & call(*)                                           \\ \hline
    \end{tabular}

\end{table}
